Automatically Mitigating Vulnerabilities in Binary Programs via Partially Recompilable Decompilation

Vulnerabilities are challenging to locate and repair, especially when source code is unavailable and binary patching is required. Manual methods are time-consuming, require significant expertise, and do not scale to the rate at which new vulnerabilities are discovered. Automated methods are an attractive alternative, and we propose Partially Recompilable Decompilation (PRD). PRD lifts suspect binary functions to source, available for analysis, revision, or review, and creates a patched binary using source- and binary-level techniques. Although decompilation and recompilation do not typically work on an entire binary, our approach succeeds because it is limited to a few functions, like those identified by our binary fault localization. We evaluate these assumptions and find that, without any grammar or compilation restrictions, 70-89% of individual functions are successfully decompiled and recompiled with sufficient type recovery. In comparison, only 1.7% of the full C-binaries succeed. When decompilation succeeds, PRD produces test-equivalent binaries 92.9% of the time. In addition, we evaluate PRD in two contexts: a fully automated process incorporating source-level Automated Program Repair (APR) methods; human-edited source-level repairs. When evaluated on DARPA Cyber Grand Challenge (CGC) binaries, we find that PRD-enabled APR tools, operating only on binaries, performs as well as, and sometimes better than full-source tools, collectively mitigating 85 of the 148 scenarios, a success rate consistent with these same tools operating with access to the entire source code. PRD achieves similar success rates as the winning CGC entries, sometimes finding higher-quality mitigations than those produced by top CGC teams. For generality, our evaluation includes two independently developed APR tools and C++, Rode0day, and real-world binaries.

==> data/abr_support.tex <==
\begin{tabular}{p{1.0cm}p{1.0cm}p{1.0cm}}
\toprule
	tool & PRD & \\
\midrule
%\rowcolor{Green}
	x86 &	\checkmark &  \\  
	x86-64 & EXT-DEC-BR & \\ 
	statically-linked & \checkmark & \\
	dynamically-linked & \checkmark & \\
	GLIBC & \checkmark & \\ 
	stripped & EXT-DEC-BR & \\ 
\midrule
	supports automated repair & \checkmark & \\
	supports manual analysis &  \checkmark & \\ 
	requires availability of control flow information & \xmark & \\
	requires symbolizing the binary & \xmark & \\
\bottomrule
\end{tabular}



==> data/cgc_table.tex <==
\begin{tabular}{lRl}
\toprule
                      DARPA CGC CB name:buggy func &  CWE IDs &                                CWE Description \\
\midrule
                        KPRCA\_00013:cgc\_infixtorpn &  CWE-193 &                               Off-by-one error \\
                                                   &  CWE-457 &                 Use of uninitialized variable  \\
\rowcolor{Gray}
        NRFIN\_00041:cgc\_parse\_sentence &   CWE-20 &                         Information disclosure \\
\rowcolor{Gray}
                                     : &  CWE-120 &     Buffer copy without Checking Size of Input \\
\rowcolor{Gray}
                                     : &  CWE-122 &                     Heap-based buffer overflow \\
\rowcolor{Gray}
                                     : &  CWE-129 &             Improper validation of array index \\
\rowcolor{Gray}
                                     : &  CWE-788 &  Access of Memory Location After End of Buffer \\
                          CROMU\_00027:cgc\_WalkTree &  CWE-787 &                            Out-of-bounds Write \\
                                                   &  CWE-476 &                       Null Pointer Dereference \\
                                                   &  CWE-195 &            Signed to Unsigned Conversion error \\
\rowcolor{Gray}
            KPRCA\_00010:cgc\_init\_track &  CWE-122 &                     Heap-based buffer overflow \\
                            KPRCA\_00009:copy\_title &  CWE-170 &                      Improper Null Termination \\
\rowcolor{Gray}
  CROMU\_00001:cgc\_list\_unread\_messages &  CWE-190 &                               Integer Overflow \\
\rowcolor{Gray}
                                     : &  CWE-131 &            Improper Calculation of Buffer Size \\
\rowcolor{Gray}
                                     : &  CWE-120 &     Buffer copy without Checking Size of Input \\
                      YAN01\_00010:main &  CWE-476 &                       Null Pointer Dereference \\
\rowcolor{Gray}
         CROMU\_00032:cgc\_parseCVFFrame &  CWE-120 &     Buffer copy without Checking Size of Input \\
                         KPRCA\_00017:cgc\_play\_game &  CWE-457 &                 Use of uninitialized variable  \\
\rowcolor{Gray}
 KPRCA\_00019:cgc\_session\_configurat... &  CWE-122 &                     Heap-based buffer overflow \\
              CROMU\_00037:cgc\_SendBroadcastMessage &  CWE-798 &                  Use of Hard-coded Credentials \\
                                                   &  CWE-131 &            Improper Calculation of Buffer Size \\
\rowcolor{Gray}
                 CADET\_00001:cgc\_check &  CWE-121 &                    Stack-based buffer overflow \\
                     KPRCA\_00073:cgc\_ReportMatches &  CWE-121 &                    Stack-based buffer overflow \\
                                                   &  CWE-787 &                            Out-of-bounds Write \\
\rowcolor{Gray}
 KPRCA\_00060:cgc\_cmd\_recv\_control\_file &  CWE-122 &                     Heap-based buffer overflow \\
                NRFIN\_00076:cgc\_rider\_health\_check &  CWE-468 &                      Incorrect Pointer Scaling \\
                                                   &  CWE-822 &                  Untrusted Pointer Dereference \\
\rowcolor{Gray}
           KPRCA\_00007:cmd\_edit\_router &  CWE-129 &             Improper validation of array index \\
                     NRFIN\_00020:cgc\_process\_notes &   CWE-20 &                         Information disclosure \\
                                                   &  CWE-129 &             Improper validation of array index \\
                                                   &  CWE-193 &                               Off-by-one error \\
\rowcolor{Gray}
     CROMU\_00010:cgc\_push\_to\_turn\_list &  CWE-467 &                use of sizeof() on pointer type \\
                       CROMU\_00033:cgc\_bubble\_sort &  CWE-125 &                             Out-of-bounds Read \\
\rowcolor{Gray}
 NRFIN\_00075:cgc\_process\_serialized... &  CWE-502 &              Deserialization of Untrusted Data \\
\rowcolor{Gray}
                                     : &  CWE-822 &                  Untrusted Pointer Dereference \\
                      NRFIN\_00035:cgc\_check\_levels &   CWE-20 &                      Improper Input Validation \\
                                                   &  CWE-128 &                              Wrap-around Error \\
                                                   &  CWE-129 &             Improper validation of array index \\
                                                   &  CWE-190 &                               Integer Overflow \\
                                                   &  CWE-788 &  Access of Memory Location After End of Buffer \\
                                                   &  CWE-805 &      Buffer Access with Incorrect Length Value \\
                                                   &  CWE-824 &                Access of Uninitialized Pointer \\
\bottomrule
\end{tabular}


==> data/complete_table.tex <==
\begin{tabular}{llllllllllllllllllllllllllllllllllllllllllllllllllllllllllllll}
\toprule
{} &                                    cb-multios name & Fn id &    POV &      CGC type &        &&&&&&&&\multicolumn{3}{P{2.8cm}{Prophet}}&\multicolumn{3}{P{2.8cm}{GenProg}}&\\
DARPA CGC CB name &                                               CWEs &  CWE IDs &                                CWE Description & Addressed CWEs & \# Addressed CWEs & \# AST nodes & \# vuln funcs & \# decompiled vuln funcs & \% vulns in PRD Decompilation &    Prophet (full) &                 GenProg (full) &  Prophet (ideal) &  GenProg (ideal) &        Prophet (PRD) &        GenProg (PRD) & Exploit Mitigated & Repair: Type 2  & Repair: Type 3 & Distinct Repairs & Total Candidates & POLL tests & Total POV tests & Valid POVs & PRD funcs & ave. statements/function &                              entry &  CB LOC & PRD LOC & rate of repair & scope reduction & \# CRS repairs &     Mayhem & Buffer copy without Checking Size of Input & Stack-based buffer overflow & Heap-based buffer overflow & Out of bounds read & Improper validation of array index & Improper Calculation of Buffer Size & Improper Null Termination & Integer Overflow & Off-by-one error & Signed to Unsigned Conversion error & Information disclosure & Use of uninitialized variable  & use of sizeof() on pointer type & Incorrect Pointer Scaling & Null Pointer Dereference & Improper Handling of Exceptional Conditions & Out-of-bounds Write & Access of Memory Location After End of Buffer & Use of Hard-coded Credentials & Untrusted Pointer Dereference & Numeric Range Comparison Without Minimum Check & Deserialization of Untrusted Data & Unnamed: 59 & Unnamed: 60 \\
\midrule
\textbf{0 } &                                              Accel &     0 &    all &     Qualifier &              KPRCA\_00013 &                                   CWE-193, CWE-457 &  CWE-193 &                               Off-by-one error &        CWE-193 &           1 of 2 &         349 &            2 &                       1 &                          0.5 &                  &                               &      &        \checkmark &                      &                      &         \checkmark &       \checkmark &                &              181 &           70,178 &         44 &               2 &          2 &                7 &                       49 &                     cgc\_infixtorpn &   2,360 &          1,917 &    0.002579156 &     0.187711864 &             3 &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &        \checkmark &                                     &                        &                          \xmark &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{1 } &                                                    &       &        &             - &                          &                                   CWE-193, CWE-457 &  CWE-457 &                 Use of uninitialized variable  &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{2 } &                                              Accel &     0 &  pov\_1 &               &              KPRCA\_00013 &                                   CWE-193, CWE-457 &          &                                                &                &                  &         349 &            2 &                       1 &                          0.5 &        \checkmark &                     \checkmark &        \checkmark &        \checkmark &            \checkmark &            \checkmark &         \checkmark &                 &                &                  &                  &         44 &               2 &          2 &                7 &                       49 &                     cgc\_infixtorpn &   2,360 &          1,917 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{3 } &                                              Accel &     0 &  pov\_2 &               &              KPRCA\_00013 &                                                    &          &                                                &                &                  &             &              &                         &                              &        \checkmark &                     \checkmark &        \checkmark &        \checkmark &            \checkmark &            \checkmark &         \checkmark &                 &                &                  &                  &            &                 &            &                  &                          &                     cgc\_infixtorpn &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{4 } &                                           AIS-Lite &     0 &  pov\_1 &     Qualifier &  ROWCOLORGRAYNRFIN\_00041 &         CWE-20, CWE-120, CWE-122, CWE-129, CWE-788 &   CWE-20 &                         Information disclosure &         CWE-20 &           5 of 5 &         207 &            1 &                       1 &                            1 &      &                     \checkmark &      &      &          &         $\perp$ &                   &                 &                &                  &           19,072 &         84 &               1 &          1 &                8 &                       25 &                 cgc\_parse\_sentence &   1,138 &            510 &              0 &     0.551845343 &             5 &  \checkmark &                                  \checkmark &                             &                  \checkmark &                    &                          \checkmark &                                     &                           &                  &                  &                                     &              \checkmark &                                &                                 &                           &                          &                                             &                     &                                     \checkmark &                               &                               &                                                &                                   &             &             \\
\textbf{5 } &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-120 &     Buffer copy without Checking Size of Input &        CWE-120 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{6 } &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-122 &                     Heap-based buffer overflow &        CWE-122 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{7 } &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-129 &             Improper validation of array index &        CWE-129 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{8 } &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-788 &  Access of Memory Location After End of Buffer &        CWE-788 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{9 } &                               ASCII\_Content\_Server &     4 &    all &     Qualifier &              CROMU\_00027 &                          CWE-787, CWE-476, CWE-195 &  CWE-787 &                            Out-of-bounds Write &        CWE-787 &           1 of 3 &         129 &            5 &                       1 &                          0.2 &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &           13,303 &        200 &               5 &          4 &                3 &                       43 &                       cgc\_WalkTree &   7,502 &             83 &              0 &     0.988936284 &             6 &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                               \xmark &                        &                                &                                 &                           &                    \xmark &                                             &           \checkmark &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{10} &                                                    &       &        &             - &                          &                          CWE-787, CWE-476, CWE-195 &  CWE-476 &                       Null Pointer Dereference &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{11} &                                                    &       &        &             - &                          &                          CWE-787, CWE-476, CWE-195 &  CWE-195 &            Signed to Unsigned Conversion error &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{12} &                               ASCII\_Content\_Server &     4 &  pov\_2 &               &              CROMU\_00027 &                          CWE-787, CWE-476, CWE-195 &          &                                                &                &                  &         129 &            5 &                       1 &                          0.2 &    $\perp$ &                   &      &      &          &          &                   &                 &                &                  &                  &        200 &               5 &          4 &                3 &                       43 &                       cgc\_WalkTree &   7,502 &             83 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{13} &                               ASCII\_Content\_Server &     4 &  pov\_3 &               &              CROMU\_00027 &                                                    &          &                                                &                &                  &             &              &                         &                              &    $\perp$ &                     \checkmark &      &      &          &          &                   &                 &                &                  &                  &            &                 &            &                  &                          &                       cgc\_WalkTree &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{14} &                               ASCII\_Content\_Server &     4 &  pov\_4 &               &              CROMU\_00027 &                                                    &          &                                                &                &                  &             &              &                         &                              &    $\perp$ &                   &      &      &          &          &                   &                 &                &                  &                  &            &                 &            &                  &                          &                       cgc\_WalkTree &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{15} &                               ASCII\_Content\_Server &     4 &  pov\_5 &               &              CROMU\_00027 &                                                    &          &                                                &                &                  &             &              &                         &                              &    $\perp$ &                   &      &      &          &          &                   &                 &                &                  &                  &            &                 &            &                  &                          &                       cgc\_WalkTree &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{16} &                                   Audio\_Visualizer &     1 &  pov\_1 &     Qualifier &  ROWCOLORGRAYKPRCA\_00010 &                                            CWE-122 &  CWE-122 &                     Heap-based buffer overflow &        CWE-122 &           1 of 1 &         185 &            2 &                       2 &                            1 &        \checkmark &                     \checkmark &      &        \checkmark &            \checkmark &          &         \checkmark &       \checkmark &                &              406 &           16,897 &         99 &               1 &          1 &               14 &                       13 &                     cgc\_init\_track &   1,920 &            744 &    0.024027934 &          0.6125 &             5 &  \checkmark &                                            &                             &                  \checkmark &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{17} &                                     basic\_emulator &     0 &    all &     Qualifier &              KPRCA\_00009 &                                            CWE-170 &  CWE-170 &                      Improper Null Termination &        CWE-170 &           1 of 1 &          11 &            1 &                       1 &                            1 &                  &                               &        \checkmark &        \checkmark &                      &                      &         \checkmark &       \checkmark &                &               72 &              230 &        100 &               3 &          3 &                3 &                        3 &                         copy\_title &   8,397 &            107 &    0.313043478 &     0.987257354 &             5 &  \checkmark &                                            &                             &                            &                    &                                    &                                     &                 \checkmark &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{18} &                                     basic\_emulator &     0 &  pov\_1 &               &              KPRCA\_00009 &                                            CWE-170 &          &                                                &                &                  &          11 &            1 &                       1 &                            1 &        \checkmark &                     \checkmark &        \checkmark &        \checkmark &            \checkmark &         $\perp$ &         \checkmark &                 &                &                  &                  &        100 &               3 &          3 &                3 &                        3 &                         copy\_title &   8,397 &            107 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{19} &                                     basic\_emulator &     0 &  pov\_2 &               &              KPRCA\_00009 &                                                    &          &                                                &                &                  &             &              &                         &                              &        \checkmark &                     \checkmark &        \checkmark &        \checkmark &            \checkmark &         $\perp$ &         \checkmark &                 &                &                  &                  &            &                 &            &                  &                          &                         copy\_title &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{20} &                                     basic\_emulator &     0 &  pov\_3 &               &              KPRCA\_00009 &                                                    &          &                                                &                &                  &             &              &                         &                              &        \checkmark &                     \checkmark &        \checkmark &        \checkmark &            \checkmark &         $\perp$ &         \checkmark &                 &                &                  &                  &            &                 &            &                  &                          &                         copy\_title &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{21} &                                    basic\_messaging &     0 &  pov\_1 &     Qualifier &  ROWCOLORGRAYCROMU\_00001 &                          CWE-190, CWE-131, CWE-120 &  CWE-190 &                               Integer Overflow &        CWE-190 &           3 of 3 &          41 &            1 &                       1 &                            1 &      &  $\perp$ &        \checkmark &        \checkmark &  + &  + &         \checkmark &       \checkmark &                &                1 &            3,230 &        101 &               1 &          1 &                3 &                       13 &           cgc\_list\_unread\_messages &  43,394 &            126 &    0.000309598 &     0.997096373 &             3 &  \checkmark &                                  \checkmark &                             &                            &                    &                                    &                           \checkmark &                           &        \checkmark &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{22} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-131 &            Improper Calculation of Buffer Size &        CWE-131 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{23} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-120 &     Buffer copy without Checking Size of Input &        CWE-120 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{24} &                                         BitBlaster &     0 &  pov\_1 &     Qualifier &              YAN01\_00010 &                                            CWE-476 &  CWE-476 &                       Null Pointer Dereference &        CWE-476 &           1 of 1 &          14 &            1 &                       1 &                            1 &      &                     \checkmark &      &        \checkmark &  + &  + &         \checkmark &       \checkmark &                &                4 &              383 &        100 &               1 &          1 &                3 &                        4 &                   main &     228 &            123 &    0.010443864 &     0.460526316 &             4 &  \checkmark &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                \checkmark &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{25} &  Cereal\_Mixup\_\_A\_Cereal\_Vending\_Machine\_Controller &     0 &  pov\_1 &  Final Sample &  ROWCOLORGRAYNRFIN\_00075 &                                   CWE-502, CWE-822 &  CWE-502 &              Deserialization of Untrusted Data &        CWE-502 &           2 of 2 &         892 &            1 &                       1 &                            1 &        \checkmark &                 $\perp$ &      \checkmark** &      \checkmark** &  + &  + &         \checkmark &                 &                &                  &                  &         87 &               1 &          1 &                1 &                          &       cgc\_process\_serialized\_input &     882 &            178 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                     \checkmark &                                                &                         \checkmark &             &             \\
\textbf{26} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-822 &                  Untrusted Pointer Dereference &        CWE-822 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{27} &                                    CGC\_File\_System &     0 &  pov\_1 &     Qualifier &              CROMU\_00033 &                                            CWE-125 &  CWE-125 &                             Out-of-bounds Read &        CWE-125 &           1 of 1 &          53 &            1 &                       1 &                            1 &      &                   &        \checkmark &        \checkmark &            \checkmark &            \checkmark &         \checkmark &                 &                &              159 &             5288 &        100 &               1 &          1 &                1 &                       53 &                    cgc\_bubble\_sort &     988 &            105 &                &                 &               &            &                                            &                             &                            &          \checkmark &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{28} &                 CGC\_Video\_Format\_Parser\_and\_Viewer &     0 &  pov\_1 &     Qualifier &  ROWCOLORGRAYCROMU\_00032 &                                            CWE-120 &  CWE-120 &     Buffer copy without Checking Size of Input &        CWE-120 &           1 of 1 &         134 &            1 &                       1 &                            1 &      &                   &        \checkmark &      &  + &  + &         \checkmark &                 &                &                  &           35,264 &        101 &               1 &          1 &                3 &                       44 &                  cgc\_parseCVFFrame &   1,151 &            313 &              0 &     0.728062554 &             3 &  \checkmark &                                  \checkmark &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{29} &                                         H20FlowInc &     0 &  pov\_1 &     Qualifier &              NRFIN\_00035 &  CWE-20, CWE-128, CWE-129, CWE-190, CWE-788, CW... &   CWE-20 &                      Improper Input Validation &                &                  &         757 &              &                         &                              &      &                     \checkmark &      &      &          &         $\perp$ &                 - &                 &                &                  &                  &        100 &               1 &          1 &                1 &                          &                   cgc\_check\_levels &    6755 &            140 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{30} &                                                    &       &        &             - &                          &                                                    &  CWE-128 &                              Wrap-around Error &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{31} &                                                    &       &        &             - &                          &                                                    &  CWE-129 &             Improper validation of array index &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{32} &                                                    &       &        &             - &                          &                                                    &  CWE-190 &                               Integer Overflow &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{33} &                                                    &       &        &             - &                          &                                                    &  CWE-788 &  Access of Memory Location After End of Buffer &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{34} &                                                    &       &        &             - &                          &                                                    &  CWE-805 &      Buffer Access with Incorrect Length Value &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{35} &                                                    &       &        &             - &                          &                                                    &  CWE-824 &                Access of Uninitialized Pointer &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{36} &                                            HackMan &     0 &    all &     Qualifier &  ROWCOLORGRAYKPRCA\_00017 &                                            CWE-457 &  CWE-457 &                 Use of uninitialized variable  &        CWE-457 &           1 of 1 &          50 &            1 &                       1 &                            1 &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &            4,970 &         29 &               2 &          2 &                3 &                       16 &                      cgc\_play\_game &   1,225 &            162 &              0 &     0.867755102 &             6 &  \checkmark &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                      \checkmark &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{37} &                                            HackMan &     0 &  pov\_1 &               &  ROWCOLORGRAYKPRCA\_00017 &                                            CWE-457 &          &                                                &                &                  &          50 &            1 &                       1 &                            1 &      &                   &      &      &          &        $\bowtie$ &                   &                 &                &                  &                  &         29 &               2 &          2 &                3 &                       16 &                      cgc\_play\_game &   1,225 &            162 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{38} &                                            HackMan &     0 &  pov\_2 &               &  ROWCOLORGRAYKPRCA\_00017 &                                                    &          &                                                &                &                  &             &              &                         &                              &        \checkmark &                   &        \checkmark &        \checkmark &            \checkmark &        $\bowtie$ &         \checkmark &                 &                &                  &                  &            &                 &            &                  &                          &                      cgc\_play\_game &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{39} &                                     humaninterface &     0 &    all &     Qualifier &              KPRCA\_00019 &                                            CWE-122 &  CWE-122 &                     Heap-based buffer overflow &        CWE-122 &           1 of 1 &          49 &            1 &                       1 &                            1 &                  &                               &        \checkmark &        \checkmark &                      &                      &         \checkmark &       \checkmark &                &              213 &            4,712 &        100 &               2 &          2 &                3 &                       16 &  cgc\_session\_configuration\_request &   1,399 &            216 &    0.045203735 &     0.845604003 &             5 &  \checkmark &                                            &                             &                  \checkmark &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{40} &                                     humaninterface &     0 &  pov\_1 &               &              KPRCA\_00019 &                                            CWE-122 &          &                                                &                &                  &          49 &            1 &                       1 &                            1 &        \checkmark &                   $\perp$ &        \checkmark &        \checkmark &  + &  + &         \checkmark &                 &                &                  &                  &        100 &               2 &          2 &                3 &                       16 &  cgc\_session\_configuration\_request &   1,399 &            216 &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{41} &                                     humaninterface &     0 &  pov\_2 &               &              KPRCA\_00019 &                                                    &          &                                                &                &                  &             &              &                         &                              &        \checkmark &                   $\perp$ &        \checkmark &        \checkmark &  + &  + &         \checkmark &                 &                &                  &                  &            &                 &            &                  &                          &  cgc\_session\_configuration\_request &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{42} &                                    Message\_Service &     0 &  pov\_1 &     Qualifier &  ROWCOLORGRAYCROMU\_00037 &                                   CWE-798, CWE-131 &  CWE-798 &                  Use of Hard-coded Credentials &        CWE-131 &           1 of 2 &          26 &            1 &                       1 &                            1 &        \checkmark &       $\perp$ &        \checkmark &        \checkmark &            \checkmark &            \checkmark &         \checkmark &       \checkmark &                &              198 &            1,307 &        101 &               1 &          1 &                3 &                        8 &           cgc\_SendBroadcastMessage &  52,123 &            124 &    0.151491966 &     0.997621012 &             6 &  \checkmark &                                            &                             &                            &                    &                                    &                           \checkmark &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                         \xmark &                               &                                                &                                   &             &             \\
\textbf{43} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-131 &            Improper Calculation of Buffer Size &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{44} &                                        Palindrome2 &     0 &  pov\_1 &        Sample &              CADET\_00001 &                                            CWE-121 &  CWE-121 &                    Stack-based buffer overflow &        CWE-121 &           1 of 1 &          33 &            1 &                       1 &                            1 &      &                     \checkmark &      &      &          &          &                   &                 &                &                  &            2,007 &         99 &               1 &          1 &                4 &                        8 &                          cgc\_check &     208 &             97 &              0 &     0.533653846 &           N/A &          - &                                            &                   \checkmark &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{45} &                                     Pattern\_Finder &     0 &  pov\_1 &         Final &  ROWCOLORGRAYKPRCA\_00073 &                                   CWE-121, CWE-787 &  CWE-121 &                    Stack-based buffer overflow &        CWE-121 &           2 of 2 &          17 &            1 &                       1 &                            1 &      &                   &        \checkmark &      &            \checkmark &         $\perp$ &         \checkmark &                 &                &                  &              557 &         93 &               1 &          1 &                3 &                        5 &                  cgc\_ReportMatches &   1,918 &            129 &              0 &      0.93274244 &           N/A &            &                                            &                   \checkmark &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &           \checkmark &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{46} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-787 &                            Out-of-bounds Write &        CWE-787 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{47} &                                            Printer &     0 &  pov\_1 &  Final Sample &              KPRCA\_00060 &                                            CWE-122 &  CWE-122 &                     Heap-based buffer overflow &        CWE-122 &           1 of 1 &          74 &            1 &                       1 &                            1 &        \checkmark &                   &        \checkmark &        \checkmark &            \checkmark &         $\perp$ &         \checkmark &                 &                &                  &           10,718 &         51 &               1 &          1 &                3 &                       24 &          cgc\_cmd\_recv\_control\_file &   1,051 &            244 &              0 &     0.767840152 &           N/A &          - &                                            &                             &                  \checkmark &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{48} &                                    Resort\_Modeller &     0 &  pov\_1 &  Final Sample &  ROWCOLORGRAYNRFIN\_00076 &                                   CWE-468, CWE-822 &  CWE-468 &                      Incorrect Pointer Scaling &        CWE-468 &           2 of 2 &           8 &            1 &                       1 &                            1 &      &                 $\perp$ &        \checkmark &        \checkmark &  + &  + &         \checkmark &       \checkmark &      \checkmark &               31 &              128 &        100 &               1 &          1 &                3 &                        2 &             cgc\_rider\_health\_check &   1,811 &             52 &      0.2421875 &     0.971286582 &           N/A &          - &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                 \checkmark &                          &                                             &                     &                                               &                               &                     \checkmark &                                                &                                   &             &             \\
\textbf{49} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-822 &                  Untrusted Pointer Dereference &        CWE-822 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{50} &                                   router\_simulator &     0 &  pov\_1 &     Qualifier &              KPRCA\_00007 &                                            CWE-129 &  CWE-129 &             Improper validation of array index &        CWE-129 &           1 of 1 &          16 &            1 &                       1 &                            1 &        \checkmark &                     \checkmark &        \checkmark &      &            \checkmark &          &         \checkmark &                 &                &                  &              512 &         32 &               2 &          1 &                3 &                        5 &                    cmd\_edit\_router &   1,631 &            111 &              0 &     0.931943593 &             3 &            &                                            &                             &                            &                    &                          \checkmark &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{51} &                                           SOLFEDGE &     0 &    all &     Qualifier &  ROWCOLORGRAYNRFIN\_00020 &                           CWE-20, CWE-129, CWE-193 &   CWE-20 &                         Information disclosure &         CWE-20 &           3 of 3 &          57 &            1 &                       1 &                            1 &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &            2,690 &         92 &               2 &          2 &                6 &                        9 &                  cgc\_process\_notes &     720 &            139 &              0 &     0.806944444 &             3 &            &                                            &                             &                            &                    &                          \checkmark &                                     &                           &                  &        \checkmark &                                     &              \checkmark &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{52} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-129 &             Improper validation of array index &        CWE-129 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{53} &                                                    &       &        &             - &             ROWCOLORGRAY &                                                    &  CWE-193 &                               Off-by-one error &        CWE-193 &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{54} &                                           SOLFEDGE &     0 &  pov\_1 &               &  ROWCOLORGRAYNRFIN\_00020 &                           CWE-20, CWE-129, CWE-193 &          &                                                &                &                  &          57 &            1 &                       1 &                            1 &      &                   &      &      &          &         $\perp$ &                   &                 &                &                  &                  &         92 &               2 &          2 &                6 &                        9 &                  cgc\_process\_notes &     720 &            139 &              0 &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{55} &                                           SOLFEDGE &     0 &  pov\_2 &               &  ROWCOLORGRAYNRFIN\_00020 &                                                    &          &                                                &                &                  &             &              &                         &                              &      &                     \checkmark &      &      &          &         $\perp$ &                   &                 &                &                  &                  &            &                 &            &                  &                          &                  cgc\_process\_notes &       - &              - &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{56} &                                 Street\_map\_service &     0 &  pov\_1 &     Qualifier &              CROMU\_00010 &                                            CWE-467 &  CWE-467 &                use of sizeof() on pointer type &        CWE-467 &           1 of 1 &           2 &            1 &                       1 &                            1 &        \checkmark &                     \checkmark &        \checkmark &      &            \checkmark &            \checkmark &                   &                 &                &                  &                8 &        100 &               1 &          1 &                1 &                        2 &              cgc\_push\_to\_turn\_list &  15,270 &            101 &              0 &     0.993385724 &             6 &  \checkmark &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                       \checkmark &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{57} &                                                    &       &        &               &                          &                                                    &          &                                                &                &                  &             &              &                         &                              &                  &                               &                  &                  &                      &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{58} &                                              Total &       &     30 &               &        ROWCOLORGRAYTotal &                                                    &          &                                                &                &                  &             &              &                         &                              &               14 &                            14 &               18 &               16 &                   13 &                    5 &                19 &               5 &              1 &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &     20.81929141 &               &            &                                          3 &                           2 &                          4 &                  1 &                                  3 &                                   2 &                         1 &                1 &                2 &                                   0 &                      2 &                              1 &                               1 &                         1 &                        1 &                                           0 &                   2 &                                             1 &                             0 &                             2 &                                              0 &                                 1 &             &             \\
\textbf{59} &                                                    &       &        &               &             ROWCOLORGRAY &                                                    &          &                                                &                &                  &             &              &                         &                              &                  &                               &                  &                  &                    7 &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\textbf{60} &                                                    &       &        &               &             ROWCOLORGRAY &                                                    &          &                                                &                &                  &             &              &                         &                              &                  &                               &                  &                  &                   10 &                      &                   &                 &                &                  &                  &            &                 &            &                  &                          &                                    &         &                &                &                 &               &            &                                            &                             &                            &                    &                                    &                                     &                           &                  &                  &                                     &                        &                                &                                 &                           &                          &                                             &                     &                                               &                               &                               &                                                &                                   &             &             \\
\bottomrule
\end{tabular}


==> data/partdecomp_eval.tex <==
\iffalse
\begin{tabular}{|p{1.75cm}|p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}|}
\hline
	DataSet & -- & Type Recovery & Decompile & Basic Recompile \\
\hline
	CGC-C & Total & 100 & 7067 & 6200 \\
	 & Failed & 8 & 877 & 1783 \\
	 & Passed & 92 & 6190 & 4417 \\
\hline
	CGC-C++ & Total & 10 & 1254 & 839 \\
& Failed & 10 & 412 & 528 \\
& Passed & 0 & 839 & 311 \\
\hline
Rode0days & Total & 4 & 3298 & 3297 \\
& Failed & 2 & 1 & 2934 \\
& Passed & 2 & 3297 & 363 \\
\hline

\end{tabular}
\else

\begin{comment}
\begin{tabular}{|p{1.75cm}|p{1.35cm}p{1.75cm}p{1.75cm}|p{1.75cm}|}
	\hline
	DataSet & Type \mbox{Recovery} & Decompile & Basic \mbox{Recompile} & Binary Reconstruction \\
	\hline
	CGC-C & 92.0\% & 87.6\% & 71.2\% & 0.0\% \\
	&  92/100 & 6190/7067 & 4417/6200 & 0/100  \\
	\hline
	CGC-C++ & 0.0\% & 67.1\% & 37.1\% & 0.0\% \\
 & 0/10 & 839/1251 & 311/839  & 0/10\\
\hline
	Rode0days & 50.0\% & 99.9\% & 30.5\% & 0.0\% \\
 & 2/4 & 3297/3298 & 1007/3297 & 0/4 \\
\hline
	
\end{tabular}
\end{comment}

\begin{comment}
\begin{tabular}{|p{1.75cm}|p{1.35cm}p{1.75cm}p{1.75cm}|}
	\hline
	DataSet & Type \mbox{Recovery} & Decompile & Basic \mbox{Recompile} \\
	\hline
	CGC-C & 92.0\% & 87.6\% & 71.2\% \\
	&  92/100 & 6190/7067 & 4417/6200 \\
	\hline
	CGC-C++ & 0.0\% & 67.1\% & 37.1\% \\
	& 0/10 & 839/1251 & 311/839 \\
	\hline
	Rode0days & 50.0\% & 99.9\% & 30.5\% \\
	& 2/4 & 3297/3298 & 1007/3297 \\
	\hline
	
\end{tabular}
\end{comment}
\begin{tabular}{|p{1.75cm}|p{1.35cm}p{1.75cm}p{1.75cm}|p{1.75cm}|}
	%\hline
	%& \multicolumn{4}{c|}{Partial decompilation} \\
	%\hline
	\hline%\toprule
	& & Success &  & Failure \\
	\hline%\midrule
	 & Type \mbox{Recovery} & Decompile & Basic \mbox{Recompile} & Incomplete Typing \\
	\hline%\midrule
	CGC-C & 92.0\% & 87.7\% & 71.2\% & 6.8\% \\
	&  92/100 & 6200/7067 & 4417/6200 & 420/6200  \\
	\hline%\midrule
	CGC-C++ & 0.0\% & 67.1\% & 37.1\% & 48.3\% \\
	& 0/10 & 839/1251 & 311/839  & 405/839\\
	\hline%\midrule
	Rode0days & 50.0\% & 100.0\% & 18.8\% & 73.6\% \\
	& 2/4 & 3295/3295 & 620/3295 & 2425/3295 \\
	%\bottomrule
	\hline
	Total & 82.5\% & 88.9\% & 51.8\% & 31.4\% \\
	%& 94/114 & 10336/11616 & 5735/10336 & 1318/10336 \\
	\hline
	
\end{tabular}

\fi

\begin{comment}
\begin{table}
	\caption{Table captions should be placed above the
		tables.}\label{tab1}
	\begin{tabular}{|l|l|l|}
		\hline
		Heading level &  Example & Font size and style\\
		\hline
		Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
		1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
		2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
		3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
		4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
		\hline
	\end{tabular}
\end{table}

\end{comment}




==> data/prd_decompile_results.tex <==
\iffalse
\begin{tabular}{p{0.65cm}p{1.0cm}p{0.85cm}p{3.2cm}Q{0.4cm}}
\toprule
	Result & Failure type & Static / dynamic & Description & Count \\
\midrule
\rowcolor{Green}
	success &  &  & test-equivalent & 4790 \\
\midrule
\rowcolor{DGray}
	failure & decompiler & static & recompilation errors & 2969 \\
\rowcolor{LGray}
	failure & decompiler & static & hex-rays failed decompilation & 1134 \\
\rowcolor{DGray}
	failure & decompiler & static & unbound or undefined symbols & 76 \\
\rowcolor{LGray}
	failure & decompiler & dynamic & inconsistent test-case results & 907 \\
%\rowcolor{LGray}
%	failure & location & dynamic & POV requires symbol location & 1\\
% note from pemma: these earlier results had two CBs that had intermittent failures with negative tests - updating with reduced set (8/3)
\bottomrule
	 TOTAL & & & & 9876 
\end{tabular}
\else
\begin{tabular}{p{0.65cm}p{0.9cm}p{3.25cm}Q{1.25cm}Q{0.55cm}}
\toprule
	Result & Static / dynamic & Description & Count (C++) & Unique\\
\midrule
\rowcolor{Green}
	success &  & test-equivalent & 4790 (23) & 2181\\
\rowcolor{LGray}
    failure & static & decompilation failed & 1134 (451) & 670\\
\rowcolor{DGray}
failure & static & recompilation errors & 3045 (809) & 423\\
%\rowcolor{CFLred}
%	failure & static & recompilation errors & 2969 (809) & 347\\
% adding the following into recompilation errors
%\rowcolor{CFLred}
%	failure & static & unbound or undefined symbols & 76 (0) & 76 \\
\rowcolor{LGray}
	failure & dynamic & inconsistent test-case results & 907 (50) & 520 \\
%\rowcolor{LGray}
%	failure & location & dynamic & POV requires symbol location & 1\\
% note from pemma: these earlier results had two CBs that had intermittent failures with negative tests - updating with reduced set (8/3)
\bottomrule
	 TOTAL & & & 9876 (1343) & 
\end{tabular}


\fi


==> data/prd_e2e_results.tex <==
\begin{tabular}{p{0.65cm}p{1.0cm}p{0.7cm}p{3.55cm}Q{0.35cm}Q{0.35cm}}
\toprule
	Result & Failure type & Static / dynamic & Description & CGC & Rode-0day \\
\midrule
\rowcolor{Green}
	success &  &  & test-equivalent & 109 & 33\\
\rowcolor{LGray}
	failure & decompiler & static & no actual function in vulnerable-set & 1 & 0\\
\rowcolor{DGray}
	failure & decompiler & static & decompilation failed & 22& 46\\
\rowcolor{LGray}
	failure & decompiler & static & recompilation errors & 31& 6 \\
\rowcolor{DGray}
	failure & decompiler & static & unbound or undefined symbols & 22& 0\\
\rowcolor{LGray}
	failure & decompiler & dynamic & functional errors in decompilation & 2 & 14\\
\rowcolor{DGray}
	failure & decompiler & dynamic & decompiler missed \_\_attribute\_\_ & 1& 0\\
\rowcolor{LGray}
	failure & c-lang & dynamic & reference is multi-dimen array & 2& 0\\
%\rowcolor{LGray}
%	failure & location & dynamic & POV requires symbol location & 1\\
% note from pemma: these earlier results had two CBs that had intermittent failures with negative tests - updating with reduced set (8/3)
\bottomrule
	 TOTAL & & & & 190 & 99
\end{tabular}



==> data/prd_e2e_results_textwidth.tex <==
\begin{tabular}{lQ{1cm}Q{0.9cm}p{5.5cm}p{0.8cm}}
\toprule
	status& failure type & static / dynamic & description & count \\
\midrule
\rowcolor{Green}
	success &  &  & executionally equivalent to original vulnerable binary & 109\\
\midrule
\rowcolor{DGray}
	fail & decompiler-related & static & recompilation failed due to compile errors & 32\\
\rowcolor{LGray}
	 & - & - & hex-rays failed during decompilation & 22\\
\rowcolor{DGray}
	 & - & - & unbound or undefined symbols & 22\\
\rowcolor{LGray}
	 & - & - & no actual function in buggy-set & 1\\
\rowcolor{DGray}
	 & - & dynamic & functional errors in decompiled content & 2\\
\rowcolor{LGray}
	 & - & - & decompiler missed specific \_\_attribute\_\_ & 1\\
\rowcolor{DGray}
	 & c-lang & dynamic & improperly referencing multi-dimensional array & 2\\
\rowcolor{LGray}
	 & memory-location & dynamic & POV-required static object memory location moved during binary rewriting & 1\\
\bottomrule
	 TOTAL & & & & 192
\end{tabular}



==> data/prd_support.tex <==
\begin{tabular}{p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}}
\toprule
	tool & x86 & x86-64 & dynamically-linked & GLIBC & supports automated repair & enables manual analysis & supports stripped binaries  \\
\midrule
%\rowcolor{Green}
	PRD & \checkmark & EXT-DEC & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & EXT-DEC \\
\midrule
\rowcolor{DGray}
	failure & decompiler & static & recompilation errors & 2969 \\
\rowcolor{LGray}
	failure & decompiler & static & hex-rays failed decompilation & 1134 \\
\rowcolor{DGray}
	failure & decompiler & static & unbound or undefined symbols & 76 \\
\rowcolor{LGray}
	failure & decompiler & dynamic & inconsistent test-case results & 907 \\
%\rowcolor{LGray}
%	failure & location & dynamic & POV requires symbol location & 1\\
% note from pemma: these earlier results had two CBs that had intermittent failures with negative tests - updating with reduced set (8/3)
\bottomrule
	 TOTAL & & & & 9876 
\end{tabular}



==> data/rode0day.cgfl_results.tex <==
\begin{tabular}{p{0.75cm}Q{0.5cm}Q{1.35cm}|Q{1.25cm}}
\toprule
 Criteria & Successes & Failures & Total
\midrule
 Target in CGFL & 156 & 50 & 206
 Decomp Results & 206 & 0 & 206
 Recomp Results & 206 & 0 & 206
 Test-Equiv & 162 & 44 & 206
 Target in Decomp & 47 & 109 & 156
\bottomrule
\end{tabular}



==> data/rode0day.prd_results.tex <==
\begin{tabular}{p{0.75cm}Q{0.5cm}|Q{1.35cm}Q{1.25cm}Q{1.25cm}|Q{1.25cm}}
\toprule
	 &  & \multicolumn{3}{c|}{Success Count} & Decomp \\
	Program & Funcs & Decomp & Recomp & Test-Equiv & type failure \\
\midrule
	fileS5 & 321 & 298 (92.8\%) & 185 (62.1\%) & 182 (98.4\%) & 23 (7.2\%)\\
	pcreB4 & 175 & 168 (96.0\%) & 112 (66.7\%) & 111 (99.1\%) & 6 (3.5\%) \\
	jpegS5 & 415 & 392 (94.5\%) & 287 (73.2\%) & 265 (92.7\%) & 23 (5.5\%) \\
	sqliteB4 & 2387 & 559 (23.4\%) & 423 (75.7\%) & 412 (97.4\%) & 1823 (76.6\%) \\
\bottomrule
	TOTAL  & 3298 & 1417 (42.97\%) & 1007 (71.1\%) & \cellcolor{Green}970 (96.3\%) & 1880 (57.0\%) \\
\end{tabular}


==> data/rode0day.results.tex <==
\begin{tabular}{p{1.0cm}Q{1.0cm}Q{1.0cm}Q{1.0cm}Q{1.0cm}Q{1.0cm}|Q{1.0cm}}
\toprule
	program & evaluated functions & passing decompilations & passing recompilations & passing inline-asm & test-equivalent & missing type \\
\midrule
	fileS5 & 321 & 321 (100\%) & 185 (58\%) & 185 (100\%) & 182 (98.4\%) & 23 (7.2\%)\\
	pcreB4 & 175 & 174 (99.4\%) & 112 (64\%) & 112 (100\%) & 111 (99.1\%) & 6 (3.5\%) \\
	jpegS5 & 415 & 415 (100\%) & 287 (69\%) & 286 (99.7\%) & 265 (92.7\%) & 23 (5.5\%) \\
	sqliteB4 & 2387 & 2387 (100\%) & 423 (18\%) & 423 (100\%) & 412 (97.4\%) & 1823 (76.6\%) \\
\bottomrule
	success rate &  & 99.97\% & 30.5\% & 99.9\% & 96.4\% & (57.0\%) \\
\end{tabular}


==> detwref_fig.tex <==
\begin{figure}[!t]

	\caption{\emph{Detouring with References}. The left identifies important input features for \BinaryManipulation, the right shows its output. Symbol resolution is indicated by orange arrows, change in control flow by black arrows.
	\vspace{-0.35cm}}
	\centerline{\includegraphics[clip,trim=0.25cm 1.8cm 0.2cm 2.0cm, width=\linewidth]{detour.pdf}}
	%pdr reduction on 4/23: Unlike \emph{Simple Detouring}, objects from original binary content are referenced.
	\label{fig:complexdet}
\end{figure}

